Dwarf Galaxies with Radio-excess AGNs in the VLA Sky Survey

We present a systematic search for radio active galactic nuclei (AGNs) in dwarf galaxies using recent observations taken by the Very Large Array Sky Survey (VLASS). To select these objects, we first establish a criterion to identify radio-excess AGNs using the infrared-radio correlation (IRRC) parameter, $q$, that describes the tight relation between radio and IR emission in star forming (SF) galaxies. We find a $2\sigma$ threshold of $q < 1.94$ to select radio-excess AGNs, which is derived from a sample of $\sim 7,000$ galaxies across the full mass range in the NASA-Sloan Atlas (NSA) that have radio and IR detections from VLASS and the Wide-Field Infrared Survey Explorer, respectively. We create catalogs of radio-excess AGNs and SF galaxies and make these available to the community. Applying our criterion to dwarf galaxies with stellar masses $M_\star \lesssim 3 \times 10^9 M_\odot$ and redshifts $z \le 0.15$, and carefully removing interlopers, we find 10 radio-excess AGNs with radio-optical positional offsets between $\sim$ 0 and 2.3 arcseconds (0 - 2.7 kpc). Based on statistical arguments and emission line diagnostics, we expect the majority of these radio-excess AGNs to be associated with the dwarf host galaxies rather than background AGNs. Five of the objects have evidence for hosting AGNs at other wavelengths, and 5 objects are identified as AGNs in dwarf galaxies for the first time. We also identify 8 variable radio sources in dwarf galaxies by comparing the VLASS epoch 1 and epoch 2 observations to FIRST detections presented in arXiv:1909.04670.

==> name.tex <==
\author{John-Michael Eberhard}
\affiliation{eXtreme Gravity Institute, Department of Physics, Montana State University, Bozeman, MT 59717, USA}
\author[0000-0001-7158-614X]{Amy E. Reines}
%\author{Amy Reines}
\affiliation{eXtreme Gravity Institute, Department of Physics, Montana State University, Bozeman, MT 59717, USA}
\author[0000-0003-1436-7658]{Hansung B. Gim}
\affiliation{eXtreme Gravity Institute, Department of Physics, Montana State University, Bozeman, MT 59717, USA}
\author[0000-0003-2511-2060]{Jeremy Darling}
\affiliation{Center for Astrophysics and Space Astronomy, Department of Astrophysical and Planetary Sciences, University of Colorado, 389 UCB, Boulder, CO 80309-0389, USA}
\author[0000-0002-5612-3427]{Jenny E. Greene}
\affiliation{Department of Astrophysical Sciences, Princeton University, Princeton, NJ
08544, USA}


\vspace{5mm}
A.E.R. gratefully acknowledges support for this work provided by NSF through CAREER award 2235277 and NASA through EPSCoR grant No. 80NSSC20M0231.
